Multi-Frequency Phase Synchronization

We propose a novel formulation for phase synchronization -- the statistical problem of jointly estimating alignment angles from noisy pairwise comparisons -- as a nonconvex optimization problem that enforces consistency among the pairwise comparisons in multiple frequency channels. Inspired by harmonic retrieval in signal processing, we develop a simple yet efficient two-stage algorithm that leverages the multi-frequency information. We demonstrate in theory and practice that the proposed algorithm significantly outperforms state-of-the-art phase synchronization algorithms, at a mild computational costs incurred by using the extra frequency channels. We also extend our algorithmic framework to general synchronization problems over compact Lie groups.

==> method.tex <==
\section{Method Overview}
\label{sec:method-overview}

The novel multi-frequency algorithmic framework we propose
in this paper for angular synchronization is inspired by the
following simple observation inspired by considerations
in \cite{BCS2015,PWBM2018}: \TG{TG: Motivate this using $k_{\mathrm{max}}=2$}

This paper stems from our
attempt to incorporate the correlation structure across noisy pairwise
measurements into the angular synchronization framework. The algorithmic
paradigm we propose leverages the Peter-Weyl perspective of
NUG differently from the AMP algorithm in
\cite{PWBM2018}. We first propose a realistic measurement model in
Section~\ref{sec:model-specification} that captures
edge-wise correlations akin to the MRA model
\eqref{eq:mra-model} but is surprisingly amenable to
theoretical analysis when transformed into the frequency
domain; the necessity of considering multiple frequencies
simultaneously becomes a natural consequence of the
realistic model rather than a model assumption for
measurements as in \cite{PWBM2018}. For
simplicity of exposition and comparison, we present in this
paper the new model with \TG{sub-?}Gaussian noise, but it is
straightforward to generalize the model to incorporate other
noise types.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "sas_icml2019"
%%% End:


==> noise_model.tex <==
\section{Noise Model}
\label{sec:model-specification}

We consider angles $\theta_1,\cdots,\theta_n\in
\mathbb{R}/2\pi$, one for each of the $n$ vertices
$v_1,\cdots,v_n$ of a measurement graph $G=\left( V,E
\right)$, as ``ground truth'' to be recovered. Each angle is
observed as a noisy version $\tilde{\theta}_i\in \left[
  0,2\pi \right)$ in practice, possibly due to measurement
or discretization error. We assume the random variable
$\tilde{\theta}_i$ follows a distribution absolutely
continuous with respect to the Haar measure on
$\mathbb{R}/2\pi$ with probability density function (p.d.f.)
$p_i:\mathbb{R}/2\pi\rightarrow \mathbb{R}$. It is very natural
and moderate to make the following \emph{peak location
  assumption} (PLA):
\begin{equation}\label{eq:pla}
    \textrm{$p_i$ is peaked at the true angle $\theta_i\in\mathbb{R}/2\pi$}\tag{PLA}
\end{equation}
We assume independence across the random measurements
$\tilde{\theta}_1,\cdots,\tilde{\theta}_n$, but the relative
alignments become correlated through the pairwise
measurements $\tilde{\theta}_{ij} =
\tilde{\theta}_i - \tilde{\theta_j}\mod 2\pi$. As is
well-known, $\tilde{\theta}_{ij}$ follows a continuous
probability distribution with a density of convolution form 
\begin{equation*}
  p_i*p_{-j} \left( \theta \right)\coloneqq\int_0^{2\pi}p_{i}\left( \alpha \right)p_j \left( \alpha-\theta \right) \mathrm{d}\alpha
\end{equation*}
where $p_{-j}$ is our notation for the p.d.f. of
$-\tilde{\theta}_j$, or equivalently $p_j$ flipped with
respect to the vertical axis and then modulo $2\pi$. The
appearance of the convolution structure naturally inspires
us to consider $\tilde{\theta}_{ij}$ in their frequency
representations: The characteristic function of the random
variable $\tilde{\theta}_{ij}$ takes a decoupled form
\begin{equation}
  \label{eq:proposed-model-pdf-fourier}
  \mathbb{E}\left[ e^{\iota t \tilde{\theta}_{ij}}
  \right]=\overline{\hat{p}_i \left( t \right)} \,\,
  \hat{p}_j \left( t \right),\quad\forall t\in \mathbb{R},
  \,\,\left( i,j \right)\in E.
\end{equation}
Therefore, if we define Hermitian random matrices $W^{\left(
    k \right)}\in\mathbb{C}^{n\times n}$, $k=1,2,\cdots,$ with entries
\begin{equation}
  \label{eq:W-tensor-defn}
  W^{\left( k \right)}_{ij}:=
  \begin{cases}
    e^{\iota k\tilde{\theta}_{ij}} & \textrm{if $\left( i,j
      \right)\in E$}\\
    0 & \textrm{otherwise}
  \end{cases}
\end{equation}
then the expectations of each $W^{\left( k \right)}$ is a
partially observed version of a rank-one matrix --- more specifically,
\begin{equation}
  \label{eq:low-expected-rank}
  \mathbb{E}\left[W^{\left( k \right)}\right]=A\circ\left(\overline{z_{\left( k \right)}z_{\left( k \right)}^{*}}\right)
\end{equation}
where $z_{\left( k \right)}=\left( \hat{p}_1 \left( k
  \right),\cdots,\hat{p}_n \left( k \right)
\right)^{\top}\in\mathbb{C}^n$, and $A\in\mathbb{R}^{n\times
n}$ is the adjacency
matrix of the observation graph $G$ defined as $A_{ij}=1$ if
$\left( i,j \right)\in E$ and $A_{ij}=0$ otherwise; $\circ$
is the Hadamard (entrywise) matrix product. Entries of
$W^{\left( k \right)}$ clearly correspond to the $k$th
frequency mode of $2\pi$-periodic signals on $\mathbb{R}$ (or equivalently the $k$th irreducible representation of $\Unitary
\left( 1 \right)$). Our algorithmic paradigm leveraging
these extra representations are thus termed
``multi-frequency angular synchronization.''

We emphasize here
that, unlike the random observation pattern commonly encountered in the context
of low-rank matrix completion \cite{CR2009,CP2010,RFP2010,CT2010,CBSW2014,DR2016}, the pattern of
\eqref{eq:low-expected-rank} is deterministically dictated
by the observation graph $G$. Fortunately, our analysis of
this model is facilitated by recent progresses in matrix
completion with deterministic patterns \cite{PBN2016,SXZ2018}.

It is now extremely tempting, under the assumption \eqref{eq:pla}, to
perform low-rank matrix recovery for each
$W^{\left(k\right)}$, obtain $\hat{p}_i \left( k \right)$,
$k=1,2,\cdots$ for each vertex $v_i$, and recover the true
angle $\theta_i$ by reading off the peak of (possibly a truncated version of) the Fourier inversion
\begin{equation*}
  p_i \left( \theta \right)=\frac{1}{2\pi}\sum_{k=-\infty}^{\infty}\hat{p}_i \left( k
  \right)e^{\iota k\theta}
\end{equation*}
in which $\hat{p}_i \left( -k
\right)=\hat{p}_i \left( k \right)$ for each negative
integer $-k\in\mathbb{Z}$. This is indeed the starting point
of the new class of algorithms we propose in this paper that
incorporate harmonic retrieval techniques into angular
synchronization. We formalize this algorithmic paradigm in Section~\ref{sec:algorithm}.

\TG{TG: emphasize here that we specialize to two particular
  instantiations of the PLA model}

\TG{TG: give motivation for algorithm 1 here!}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "sas_icml2019"
%%% End:

